Learning Globally Smooth Functions on Manifolds

Smoothness and low dimensional structures play central roles in improving generalization and stability in learning and statistics. This work combines techniques from semi-infinite constrained learning and manifold regularization to learn representations that are globally smooth on a manifold. To do so, it shows that under typical conditions the problem of learning a Lipschitz continuous function on a manifold is equivalent to a dynamically weighted manifold regularization problem. This observation leads to a practical algorithm based on a weighted Laplacian penalty whose weights are adapted using stochastic gradient techniques. It is shown that under mild conditions, this method estimates the Lipschitz constant of the solution, learning a globally smooth solution as a byproduct. Experiments on real world data illustrate the advantages of the proposed method relative to existing alternatives.

==> ICML 2023 - Learning Globally Smooth Functions on Manifolds-2/alejandro_intro.tex <==
% !TEX root = main.tex
\section{Introduction}

Learning smooth functions has been shown to be advantageous in general and is of particular interest in physical systems. This is because of the general observation that close input features tend to be associated with close outputs and of the particular fact that in physical systems, Lipschitz continuity of input-output maps translates to stability and safety \citep{oberman2018lipschitz, finlay2018improved,couellan2021coupling, finlay2018lipschitz, pauli2021training, krishnan2020lipschitz, shi2019neural, lindemann2021learning, arghal2021robust}. 

To learn smooth functions one can require the parameterization to be smooth. Such is the idea, e.g., of spectral normalization of weights in neural networks \citep{miyato2018spectral, zhao2020spectral}. Smooth parameterizations have the advantage of being globally smooth, but they may be restrictive because they impose smoothness for inputs that are not necessarily realized in the data. This drawback motivates the use of Lipschitz \textit{penalties} in risk minimization \citep{oberman2018lipschitz, finlay2018improved, couellan2021coupling, pauli2021training, bungert2021clip}, which offers the opposite tradeoff. Since penalties encourage but do not enforce small Lipschitz constants, we may learn functions that are smooth on average, but with no global guarantees of smoothness at every point in the support of the data~\citep{bubeck2021a,bubeck2021law}. Formulations that guarantee \emph{global} smoothness can be obtained if the risk minimization problem is modified by the addition of a Lipschitz constant \textit{constraint} \citep{krishnan2020lipschitz, shi2019neural, lindemann2021learning, arghal2021robust}. This yields formulations that guarantee Lipschitz smoothness in all possible inputs without the drawback of enforcing smoothness outside of the input data distribution. 
%The advantage of imposing global smoothness constraints only on observed inputs is empirically attested \citep{krishnan2020lipschitz, shi2019neural, lindemann2021learning, arghal2021robust}. 
Several empirical studies \citep{krishnan2020lipschitz, shi2019neural, lindemann2021learning, arghal2021robust} demonstrated the advantage of imposing global smoothness constraints on observed inputs.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
	\centering
		\begin{subfigure}[b]{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/toy_example/1ConnectedComponent/laplacian0_05.pdf}
		%  \caption{Dataset.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/toy_example/1ConnectedComponent/lambdasbest100_014215.pdf}
		%  \caption{Manifold Lipschitz.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/toy_example/1ConnectedComponent/outputbest100_01646.pdf}
		%  \caption{Manifold Lipschitz.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/toy_example/1ConnectedComponent/output4600_ambient_1connected.pdf}
		%  \caption{Manifold Lipschitz.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/toy_example/2ConnectedComponent/laplacian0_1.pdf}
		\caption{\tiny Dataset\label{subfig:dataset}}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/toy_example/2ConnectedComponent/lambdasbest100_013376.pdf}
		\caption{\tiny Manifold Lipschitz (ours)}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/toy_example/2ConnectedComponent/outputbest90_7582.pdf}
		\caption{\tiny Manifold Regularization}
	\end{subfigure} 
	\hfill
	\begin{subfigure}[b]{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/toy_example/2ConnectedComponent/output10000_ambient2_connected.pdf}
		\caption{\tiny Ambient Regularization}
	\end{subfigure} 
	\caption{Two moons dataset. The setting consists of a two dimensional classification problem of two classes with $1$ labeled, and $200$ unlabeled samples per class. The objective is to correctly classify the $200$ unlabeled samples. We consider two cases (top) the estimated manifold has two connected components, and (bottom) the manifold is weakly connected (cf. Figure \ref{fig:two_moons}). We plot the output of a one layer neural network trained using Manifold Regularization, Manifold/Ambient Lipschitz.
	}
	\label{fig:two_moons}
\end{figure*}

In this paper we 
%observe
exploit the fact
that data can be often modeled as 
%points of a 
points in a low-dimensional
manifold. 
We therefore consider manifold Lipschitz constants in which function smoothness is assessed with respect to distances measured over the data manifold (Definition \ref{def_manifold_lipschitz}). Although this looks like a minor difference, controlling Lipschitz constants over data manifolds is quite different from controlling Lipschitz constants in the ambient space. In Figure \ref{fig:two_moons}, we look at a classification problem with classes arranged in two separate half moons. Constraining Lipschitz constants in the ambient space effectively assumes the underlying data is uniformly distributed in space [cf. Figure \ref{fig:two_moons}(d)]. Constraining Lipschitz constants in the data manifold, however, properly accounts for the data distribution [cf. Figure \ref{fig:two_moons}(a)]. 

This example also illustrates how constraining manifold Lipschitz constants is related to manifold regularization \citep{belkin2005manifold, niyogi2013manifold, li2022neural}. The difference is that manifold regularization penalizes the average norm of the manifold gradient. This distinction is significant because regularizing is more brittle than imposing constraints. In the example in Figure \ref{fig:two_moons}, manifold regularization fails to separate the dataset when the moons are close [cf. Figure \ref{fig:two_moons}-(c), bottom]. Classification with a manifold Lipschitz constant constraint is more robust to this change in the data distribution [cf. Figure \ref{fig:two_moons}-(a), bottom]. 

The advantages of constraining Lipschitz constants on manifolds that we showcase in the synthetic example of Figure \ref{fig:two_moons} manifest in the wild. To illustrate it, we empirically demonstrate this fact with two physical experiments. The first experiment entails learning a model for a differential drive ground robot in a mix of complex terrains. The second experiment consists of learning a dynamical model for a quadrotor. In both of these experiments constraining Lipschitz constants on manifolds improves upon standard risk minimization, manifold regularization, and the imposition of Lipschitz constraints in ambient space.

Global constraints on the manifold gradient yield a statistical constrained learning problem with an infinite and dense number of constraints. This is a challenging problem to approximate and solve. Here, we approach the solution of this problem in the Lagrangian dual domain and establish connections with manifold regularization that allow for the use of point cloud Laplacians. Our contributions include:


%\begin{list}
%{}
%       {
%	          \setlength{\labelwidth}{26pt}
%	          \setlength{\labelsep}{-3pt}
%	          \setlength{\itemsep}{5pt}
%	          \setlength{\leftmargin}{26pt}
%	          \setlength{\rightmargin}{0pt}
%	          \setlength{\itemindent}{0pt} 
%	          \let\makelabel=\makeboxlabel
%	       }
%\item[(C1)] 
%\item[(C2)] 
%\item [(C3)] 
%\item [(C4)] 
%\item[(C5)] 
%\end{list}

\begin{enumerate}[leftmargin=25pt,label=(C\arabic*)]
\item We introduce a constrained statistical risk minimization problem in which we learn a function that: (i) attains a target loss and (ii) attains the smallest possible manifold Lipschitz constant among functions that achieve this target loss (Section \ref{sec_problem_formulation}).

\item We introduce the Lagrangian dual problem and show that its empirical version is a statistically consistent approximation of the primal. These results do \emph{not} require the learning parametrization to be linear (Section \ref{sec_empirical_dual}).

\item We generalize results from the manifold regularization literature to show that under regularity conditions, the evaluation of manifold Lipschitz constants can be recast in a more amenable form utilizing a weighted point cloud Laplacian (Proposition \ref{P:pointcloud} in Section \ref{sec_laplacian}). 

\item We present a dual ascent algorithm to find optimal multipliers. The function that attains the target loss and minimizes the manifold Lipschitz constant follows as a byproduct (Section \ref{subsec:dual_ascent}).

\item We illustrate the merits of learning with global manifold smoothness guarantees with respect to ambient space and standard manifold regularization through two physical experiments: (i) learning model mismatches in differential drive steering over non-ideal surfaces and (ii) learning the motion dynamics of a quadrotor  (Section \ref{sec_numerical_results}).

%\item Learning robot navigation policies in a space with obstacles and learning model mismatches in differential drive steering over non-ideal surfaces illustrate the merits of learning with global manifold smoothness guarantees with respect to ambient space and standard manifold regularization (Section \ref{sec_numerical_results}).
\end{enumerate}





==> ICML 2023 - Learning Globally Smooth Functions on Manifolds-2/juan_intro.tex <==

\section{Introduction}

Machine learning has become an ubiquitous technique to learn functions able to predict, adapt, or model different phenomena in the domains of robotics, image classification, biology, and medicine to name a few. Its success, is largely attributed to their ability to identify low-dimensional patterns in high-dimensional data. Smoothness is an appealing property of these functions, even more so if the function varies slowly over the data distribution, which often is supported on a low-dimensional structure. Smoothness improves generalization, as input features that are close tend to be associated with outputs that are close as well. Smoothness can be quantified by Lipschitz constant, which captures in the case of differentiable functions, the maximum norm of the gradient. In the particular case of physical systems smoothness is not just appealing but outright necessary. This is because Lipschitz continuity of input-output maps translates to stability and safety considerations \cite{oberman2018lipschitz, finlay2018improved,couellan2021coupling, finlay2018lipschitz, pauli2021training, shi2019neural, lindemann2021learning, arghal2021robust}. 

However appealing, learning smooth functions is a challenging endeavor given that the data distributions are unknown, and the low-dimensional distance between samples not trivial to compute (e.g. perceptual distances). Some works circumvent these obstacle by requiring the parameterization itself to be smooth. Such is the idea, e.g., of spectral normalization of weights in neural networks \cite{miyato2018spectral,zhao2020spectral}. Smooth parameterizations have the advantage of being globally smooth, and easier to implement. However, by ignoring the distribution of the data, the obtained solutions are too restrictive. This motivates another line of work, which introduces a Lipschitz constant penalty in the risk minimization problem \cite{oberman2018lipschitz, finlay2018improved, couellan2021coupling, pauli2021training, bungert2021clip}. Penalties discourage large Lipschitz constants but offer no guarantee on the Lipschitz constant of the final solution. To obtain global guarantees, the risk minimization problem is modified by the addition of a Lipschitz constant constraint only on the observed inputs \cite{krishnan2020lipschitz, shi2019neural, lindemann2021learning, arghal2021robust}. These works either solve the optimization problem unconstrained and then verify its Lipschitz constant, or utilize surrogates of the max norm. Empirical evaluations confirm the relative advantages of imposing global smoothness only on observed inputs \cite{krishnan2020lipschitz, shi2019neural, lindemann2021learning, arghal2021robust}. 

% Juan's notes on citations: 
% \cite{oberman2018lipschitz,finlay2018improved} is adds a penalty term on the lagrangian

Motivated by exploiting the low dimensional structure of the data, the areas of semi-supervised learning and manifold regularization seek to find solutions that vary slowly over the samples. In this works, an average Lipschitz constant penalty is added (i.e. the integral of the Lipschitz constant over the data). Leveraging differential geometry, by virtue of Green's identity, this integral can be calculated in a more amenable way by computing the point-cloud Laplacian over the data. However, solutions where the Lipschitz constant is controlled on average lack \emph{global} guarantees. 

In this work, we introduce a constrained learning formulation, that imposes global Lipschitz constants over the low dimensional data distribution, while requiring the function to attain a controllable performance. That is, among all the functions that probably obtain an expected loss, our formulation seeks to obtain the smoothness one dimensional data structure. By Lagrange duality, our formulation leads to an interesting observation, imposing global Lipschitz constrains, is analogous to minimizing a dynamically re-weighted Laplacian, where the dynamics are govern by the dual variables of our optimization problem. This paper provides the following contributions:  
\begin{enumerate}
    \item We formulate risk minimization problems in which learned functions attain a target loss while having the smallest possible manifold Lipschitz constant (Section \ref{sec_problem_formulation}).
    \item We show that minimizing Lipschitz constants is equivalent to a manifold regularization problem with a re-sampled data distribution. This distribution is a Lagrange multiplier function that determines the difficulty of controlling the Lipschitz constant at different points (Section \ref{sec_algorithm}).
    \item We present a dual ascent algorithm to find optimal multipliers. The function that attains the target loss and minimizes the manifold Lipschitz constant follows as a byproduct (Section \ref{sec_dual_ascent}).
\end{enumerate}

==> ICML 2023 - Learning Globally Smooth Functions on Manifolds-2/latex_resources/my_sections.tex <==
\usepackage{needspace}

% \nbsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsection}[1]{\needspace{1\baselineskip}\color{white}\medskip\subsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsection\quad #1.}}



% \nbsubsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsubsection}[1]{\needspace{1\baselineskip}\color{white}\subsubsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsubsection. #1.}}

% \myparagraph provides a paragraph title in italics. 
\newcommand{\myparagraph}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}}

% \myindenetedparagraph provides an indented paragraph with title in italics.
\newcommand{\myindentedparagraph}[1]{\needspace{1\baselineskip}\medskip \hangindent=11pt \hangafter=0 \noindent{\it #1.}}

% \myparagraphtc provides a paragraph title in italics. It adds an enter to the table of contents
\newcommand{\myparagraphtc}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}\addcontentsline{toc}{subsubsection}{\qquad\qquad\quad#1}}



==> ICML 2023 - Learning Globally Smooth Functions on Manifolds-2/latex_resources/plot_appearance.tex <==


% This command sets the appearance of axis on pgfplots
\pgfplotsset{ ylabel near ticks,                 % Make x axis label appear close to figure
              xlabel near ticks,                 % Make y axis label appear close to figure
              tick label style = {font=\tiny},   % Write numbers in tiny font
              label style = {font=\tiny},        % Write axes labels in tiny size font
              title style = {font=\tiny},        % Write figure titles in tiny size font
            }

% style to draw dots in comb plots 
\tikzstyle{dot}          =[circle, draw=none, inner sep=0pt, minimum size =1.5mm, fill=black]
\tikzstyle{red dot}      =[dot, fill=red]
\tikzstyle{blue dot}     =[dot, fill=blue ]
\tikzstyle{red blue dot} =[dot, draw, thick, minimum size =1.2mm, red, fill=blue]
\def \greenfill {mygreen!40}

==> ICML 2023 - Learning Globally Smooth Functions on Manifolds-2/oldSection2.tex <==
\section{Global Constraining of Manifold Lipschitz Constants}\label{sec_problem_formulation}

We consider data pairs $(x,y)$ in which the input features $x\in \ccalM \subset \reals^N$ 
lie in a compact oriented Riemannian manifold $\ccalM$ and the output features are real valued $y\in\reals$. We study the regression problem of finding a function \blue{$f_\theta:\ccalM \to \reals$, parameterized by $\theta\in\Theta\subset\reals^Q$} that minimizes the expectation of a nonnegative loss $\ell:\reals\times\reals\to\reals_+$, where \blue{$\ell(f_\theta(x),y)$} represent the loss of predicting output \blue{$f_\theta(x)$} when the world realizes the pair $(x,y)$. Data pairs $(x,y)$ are drawn according to an unknown probability distribution $p(x,y)$ on $\ccalM \times \reals$ which we can factor as  $p(x,y)=p(x)p(y|x)$.

We are interested in learning functions with \emph{controlled} variability over the manifold $\ccalM$. We therefore let \blue{$\nabla_\ccalM f_\theta(x)$} represent the manifold gradient of \blue{$f_\theta$} and introduce the following definition. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}[Manifold Lipschitz Constant]\label{def_manifold_lipschitz}
	Given a Riemannian manifold, $(\ccalM,d_{\ccalM})$, the function \blue{$f_\theta : \ccalM \to \reals$} is said to be $L$-Lipschitz continuous if there exists a strictly positive constant $L>0$ such that for all pairs of points $x_1,x_2 \in \ccalM$, 
	%
	\begin{align}\label{eqn_def_manifold_lipschitz_10}
		|f_\theta(x_1)-f_\theta(x_2)| \leq L\, d_{\ccalM} (x_1,x_2),
	\end{align}
	%
	where $d_\ccalM (x_1,x_2)$ denotes the metric distance between $x_1$ and $x_2$ in the manifold $\ccalM$. If the function $f_\theta$ is differentiable, \eqref{eqn_def_manifold_lipschitz_10} is equivalent to requiring the gradient norm to be bounded by $L$,
	%
	\begin{align}\label{eqn_def_manifold_lipschitz_20}
		\| \nabla_\ccalM f_\theta(x) \| 
		~ =  ~ \lim_{\delta \to 0} ~
		\sup_{ x' \neq x ~:~ d_\ccalM (x,x') \leq \delta} ~
		\frac{|f_\theta(x)-f_\theta(x')|}{d_\ccalM(x,x')}  ~
		~ \leq ~ L , \text{\quad for all~}  x \in \ccalM.
	\end{align}
	%
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

With definition \ref{def_manifold_lipschitz} in place and restricting attention to differentiable functions $f_\theta$ our stated goal of learning functions $f_\theta$ with controlled variability over the manifold $\ccalM$ can then be written as
%
% \begin{align}\label{prob:manifold_lipschitz}
	%   \underset{\phi,\rho\geq 0}{\minimize}  \quad   
	%       & \rho, \\
	%   \text{subject to}  \quad 
	%       & \mbE_{p(x,y)} [\ell \left(\phi(x),y\right)]\leq \epsilon, \nonumber\\
	%       & \| \nabla_\ccalM \phi(z) \|^2 \leq \rho ,\quad z \in \ccalM . \nonumber
	% \end{align}
\begin{align}\label{prob:manifold_lipschitz}
	P^* = \ \ \ \ \ \ \underset{\theta\in\Theta,\rho\geq 0}{\min}  \quad   
	& \rho, \\
	\text{subject to}  \quad 
	& \mbE_{p(x,y)} [\ell \left(f_\theta(x),y\right)]\leq \epsilon, \nonumber\\
	& \| \nabla_\ccalM f_\theta(z) \|^2 \leq \rho ,\quad p(z)\text{-a.e.}, \quad z \in \ccalM . \nonumber
\end{align}
%
In this formulation the statistical loss $\mbE_{p(x,y)} [\ell \left(f_\theta(x),y\right)]$ is required to be below a target level $\eps$. Of all functions $f_\theta$ that can satisfy this loss requirement, Problem \eqref{prob:manifold_lipschitz} defines as optimal the one whose Lipschitz constant $L=\sqrt{\rho}$ is smallest. The goal of this paper is to develop methodologies to solve \eqref{prob:manifold_lipschitz} when the data distribution and the manifold are unknown. To characterize the distribution we are given sample pairs $(x_i,y_i)$ drawn from the joint distribution $p(x,y)$. To characterize the manifold we are given samples $z_i$ drawn from the marginal distribution $p(x)$. This includes the samples $x_i$ from the (labeled) data pairs  $(x_i,y_i)$ and may also include (unlabeled) samples $z_i$.

It is interesting to observe that \eqref{prob:manifold_lipschitz} shows that the problems of manifold regularization \cite{belkin2005manifold, niyogi2013manifold, kejani2020graph, li2022neural} and Lipschitz constant control \cite{oberman2018lipschitz, finlay2018improved,couellan2021coupling, finlay2018lipschitz, pauli2021training, krishnan2020lipschitz, shi2019neural, lindemann2021learning, arghal2021robust} are related. This connection is important to understand the merit of \eqref{prob:manifold_lipschitz}. To explain this better observe that there are three motivations for the problem formulation in \eqref{prob:manifold_lipschitz}: (i) It is often the case that if samples $x_1$ and $x_2$ are close, then the conditional distributions $p(y|x_1)$ and $p(y|x_2)$ are close as well. A function $f_\theta$ with small Lipschitz constant leverages this property. (ii) The Lipschitz constant of $f_\theta$ is \emph{guaranteed} to be smaller than $L=\sqrt{\rho}$. This provides advantages in, e.g., physical systems where Lipschitz constant guarantees translates to stability and safety assurances. (iii) It leverages the intrinsic low-dimensional structure of the manifold $\ccalM$. In particular, this permits taking advantage of unlabeled data. 

Motivations (i) and (ii) are tropes of the Lipschitz regularization literature; e.g., \cite{oberman2018lipschitz, finlay2018improved,couellan2021coupling, finlay2018lipschitz, pauli2021training, krishnan2020lipschitz, shi2019neural, lindemann2021learning, arghal2021robust}. Indeed, the problem formulation in \eqref{prob:manifold_lipschitz} is inspired in similar problem formulations in which the Lipschitz constant is regularized in the ambient space,
%
\begin{align}\label{prob:ambient_lipschitz}
	\underset{\theta\in\Theta,\rho\geq 0}{\minimize}  \quad   
	& L, \\
	\text{subject to}  \quad 
	& \mbE_{p(x,y)} [\ell \left(f_\theta(x),y\right)]\leq \epsilon, \nonumber\\
	&  |f_\theta(y)-f_\theta(z)| \leq L\, \| y - z \|, \quad (y , z)\sim p(x) . \nonumber
\end{align}
%
A difference between \eqref{prob:manifold_lipschitz} and \eqref{prob:ambient_lipschitz} is that in the latter we use a Lipschitz condition that does not require differentiability. A more important difference is that in \eqref{prob:ambient_lipschitz} the Lipschitz constant is regularized in the ambient space. The distance between features $y$ and $z$ in \eqref{prob:ambient_lipschitz} is the Euclidean distance $\| y - z \|$. This is disparate from the manifold metric $d_\ccalM(y,z)$ that is implicit in the manifold gradient constraint in \eqref{prob:manifold_lipschitz}. Thus, the formulation in \eqref{prob:manifold_lipschitz} improves upon \eqref{prob:ambient_lipschitz} because of its ability to leverage the structure of the manifold $\ccalM$ [cf. Motivation (iii)].

Motivations (i) and (iii) are themes of the manifold regularization literature \cite{belkin2005manifold, niyogi2013manifold, kejani2020graph, li2022neural}. And, indeed, it is ready to conclude by invoking Green's first identity (see Section \ref{sec_algorithm}) that the formulation in \eqref{prob:manifold_lipschitz} is also inspired in the manifold regularization problem,
%
\begin{align}\label{prob:manifold_regularization}
	\underset{\theta\in\Theta}{\minimize}  \quad  
	\mbE_{p(x,y)} [\ell \left(f_\theta(x),y\right)] 
	+ \gamma \int_\ccalM \| \nabla_\ccalM f_\theta(z) \|^2 p(z) dV(z).
\end{align}
%
The difference between \eqref{prob:manifold_lipschitz} and \eqref{prob:manifold_regularization} is that in the latter the manifold Lipschitz constant is added as a regularization penalty. This is disparate from the imposition of a manifold Lipschitz constraint in \eqref{prob:manifold_lipschitz}. The regularization in \eqref{prob:manifold_regularization}  \emph{favors} solutions with small Lipschitz constant by penalizing large Lipschitz constants, while the constraint in \eqref{prob:manifold_lipschitz}  \emph{guarantees} that the Lipschitz constant is bounded by $\rho$. This is the distinction between \emph{regularizing} a Lipschitz constant versus \emph{constraining} a Lipschitz constant. The constraint in \eqref{prob:manifold_regularization} is also imposed at \emph{all} points in the manifold, whereas the regularization in \eqref{prob:manifold_regularization} is an average over the manifold. Taking an average allows for large Lipschitz constants at some specific points if this is canceled out by small Lipschitz constants in other points of the manifold. Both of these observations imply that \eqref{prob:manifold_lipschitz} improves upon \eqref{prob:manifold_regularization} because it offers global smoothness guarantees that are important in, e.g., physical systems [cf. Motivation (iii)].

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   R   E   M   A   R   K   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{remark}[Alternative Manifold Lipschitz Control Formulations] \normalfont
	There are three arbitrary choices in \eqref{prob:manifold_lipschitz}. (a) We choose to constrain the average statistical loss $\mbE_{p(x,y)} [\ell \left(f_\theta(x),y\right)]\leq \epsilon$; (b) we choose to constrain the pointwise Lipschitz constant $\| \nabla_\ccalM f_\theta(z) \|^2 \leq \rho$; and (c) we choose as our objective to require a target loss $\eps$ and minimize the Lipschitz constant $L=\sqrt{\rho}$. We can alternatively choose to constrain the pointwise loss $\ell \left(f_\theta(x),y\right)\leq \epsilon$, to constrain the average Lipschitz constant $\int_\ccalM \| \nabla_\ccalM f_\theta(z) \|^2 p_x(z) dV(z) \leq \rho$ [cf \eqref{prob:manifold_regularization}], or to require a target smoothness $L=\sqrt{\rho}$ and minimize the loss $\eps$. All of the possible eight combinations of choices are of interest. We formulate \eqref{prob:manifold_lipschitz} because it is the most natural intersection between the regularization of Lipschitz constants in ambient spaces [cf. \eqref{prob:ambient_lipschitz}] and manifold regularization [cf. \eqref{prob:manifold_regularization}]. The techniques we develop in this paper can be adapted to any of the other seven alternative formulations.
\end{remark}


==> juan_intro.tex <==

\section{Introduction}

Machine learning has become an ubiquitous technique to learn functions able to predict, adapt, or model different phenomena in the domains of robotics, image classification, biology, and medicine to name a few. Its success, is largely attributed to their ability to identify low-dimensional patterns in high-dimensional data. Smoothness is an appealing property of these functions, even more so if the function varies slowly over the data distribution, which often is supported on a low-dimensional structure. Smoothness improves generalization, as input features that are close tend to be associated with outputs that are close as well. Smoothness can be quantified by Lipschitz constant, which captures in the case of differentiable functions, the maximum norm of the gradient. In the particular case of physical systems smoothness is not just appealing but outright necessary. This is because Lipschitz continuity of input-output maps translates to stability and safety considerations \cite{oberman2018lipschitz, finlay2018improved,couellan2021coupling, finlay2018lipschitz, pauli2021training, shi2019neural, lindemann2021learning, arghal2021robust}. 

However appealing, learning smooth functions is a challenging endeavor given that the data distributions are unknown, and the low-dimensional distance between samples not trivial to compute (e.g. perceptual distances). Some works circumvent these obstacle by requiring the parameterization itself to be smooth. Such is the idea, e.g., of spectral normalization of weights in neural networks \cite{miyato2018spectral,zhao2020spectral}. Smooth parameterizations have the advantage of being globally smooth, and easier to implement. However, by ignoring the distribution of the data, the obtained solutions are too restrictive. This motivates another line of work, which introduces a Lipschitz constant penalty in the risk minimization problem \cite{oberman2018lipschitz, finlay2018improved, couellan2021coupling, pauli2021training, bungert2021clip}. Penalties discourage large Lipschitz constants but offer no guarantee on the Lipschitz constant of the final solution. To obtain global guarantees, the risk minimization problem is modified by the addition of a Lipschitz constant constraint only on the observed inputs \cite{krishnan2020lipschitz, shi2019neural, lindemann2021learning, arghal2021robust}. These works either solve the optimization problem unconstrained and then verify its Lipschitz constant, or utilize surrogates of the max norm. Empirical evaluations confirm the relative advantages of imposing global smoothness only on observed inputs \cite{krishnan2020lipschitz, shi2019neural, lindemann2021learning, arghal2021robust}. 

% Juan's notes on citations: 
% \cite{oberman2018lipschitz,finlay2018improved} is adds a penalty term on the lagrangian

Motivated by exploiting the low dimensional structure of the data, the areas of semi-supervised learning and manifold regularization seek to find solutions that vary slowly over the samples. In this works, an average Lipschitz constant penalty is added (i.e. the integral of the Lipschitz constant over the data). Leveraging differential geometry, by virtue of Green's identity, this integral can be calculated in a more amenable way by computing the point-cloud Laplacian over the data. However, solutions where the Lipschitz constant is controlled on average lack \emph{global} guarantees. 

In this work, we introduce a constrained learning formulation, that imposes global Lipschitz constants over the low dimensional data distribution, while requiring the function to attain a controllable performance. That is, among all the functions that probably obtain an expected loss, our formulation seeks to obtain the smoothness one dimensional data structure. By Lagrange duality, our formulation leads to an interesting observation, imposing global Lipschitz constrains, is analogous to minimizing a dynamically re-weighted Laplacian, where the dynamics are govern by the dual variables of our optimization problem. This paper provides the following contributions:  
\begin{enumerate}
    \item We formulate risk minimization problems in which learned functions attain a target loss while having the smallest possible manifold Lipschitz constant (Section \ref{sec_problem_formulation}).
    \item We show that minimizing Lipschitz constants is equivalent to a manifold regularization problem with a re-sampled data distribution. This distribution is a Lagrange multiplier function that determines the difficulty of controlling the Lipschitz constant at different points (Section \ref{sec_algorithm}).
    \item We present a dual ascent algorithm to find optimal multipliers. The function that attains the target loss and minimizes the manifold Lipschitz constant follows as a byproduct (Section \ref{sec_dual_ascent}).
\end{enumerate}

==> latex_resources/my_sections.tex <==
\usepackage{needspace}

% \nbsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsection}[1]{\needspace{1\baselineskip}\color{white}\medskip\subsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsection\quad #1.}}



% \nbsubsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsubsection}[1]{\needspace{1\baselineskip}\color{white}\subsubsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsubsection. #1.}}

% \myparagraph provides a paragraph title in italics. 
\newcommand{\myparagraph}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}}

% \myindenetedparagraph provides an indented paragraph with title in italics.
\newcommand{\myindentedparagraph}[1]{\needspace{1\baselineskip}\medskip \hangindent=11pt \hangafter=0 \noindent{\it #1.}}

% \myparagraphtc provides a paragraph title in italics. It adds an enter to the table of contents
\newcommand{\myparagraphtc}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}\addcontentsline{toc}{subsubsection}{\qquad\qquad\quad#1}}



==> latex_resources/plot_appearance.tex <==


% This command sets the appearance of axis on pgfplots
\pgfplotsset{ ylabel near ticks,                 % Make x axis label appear close to figure
              xlabel near ticks,                 % Make y axis label appear close to figure
              tick label style = {font=\tiny},   % Write numbers in tiny font
              label style = {font=\tiny},        % Write axes labels in tiny size font
              title style = {font=\tiny},        % Write figure titles in tiny size font
            }

% style to draw dots in comb plots 
\tikzstyle{dot}          =[circle, draw=none, inner sep=0pt, minimum size =1.5mm, fill=black]
\tikzstyle{red dot}      =[dot, fill=red]
\tikzstyle{blue dot}     =[dot, fill=blue ]
\tikzstyle{red blue dot} =[dot, draw, thick, minimum size =1.2mm, red, fill=blue]
\def \greenfill {mygreen!40}

==> oldSection2.tex <==
\section{Global Constraining of Manifold Lipschitz Constants}\label{sec_problem_formulation}

We consider data pairs $(x,y)$ in which the input features $x\in \ccalM \subset \reals^N$ 
lie in a compact oriented Riemannian manifold $\ccalM$ and the output features are real valued $y\in\reals$. We study the regression problem of finding a function \blue{$f_\theta:\ccalM \to \reals$, parameterized by $\theta\in\Theta\subset\reals^Q$} that minimizes the expectation of a nonnegative loss $\ell:\reals\times\reals\to\reals_+$, where \blue{$\ell(f_\theta(x),y)$} represent the loss of predicting output \blue{$f_\theta(x)$} when the world realizes the pair $(x,y)$. Data pairs $(x,y)$ are drawn according to an unknown probability distribution $p(x,y)$ on $\ccalM \times \reals$ which we can factor as  $p(x,y)=p(x)p(y|x)$.

We are interested in learning functions with \emph{controlled} variability over the manifold $\ccalM$. We therefore let \blue{$\nabla_\ccalM f_\theta(x)$} represent the manifold gradient of \blue{$f_\theta$} and introduce the following definition. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}[Manifold Lipschitz Constant]\label{def_manifold_lipschitz}
	Given a Riemannian manifold, $(\ccalM,d_{\ccalM})$, the function \blue{$f_\theta : \ccalM \to \reals$} is said to be $L$-Lipschitz continuous if there exists a strictly positive constant $L>0$ such that for all pairs of points $x_1,x_2 \in \ccalM$, 
	%
	\begin{align}\label{eqn_def_manifold_lipschitz_10}
		|f_\theta(x_1)-f_\theta(x_2)| \leq L\, d_{\ccalM} (x_1,x_2),
	\end{align}
	%
	where $d_\ccalM (x_1,x_2)$ denotes the metric distance between $x_1$ and $x_2$ in the manifold $\ccalM$. If the function $f_\theta$ is differentiable, \eqref{eqn_def_manifold_lipschitz_10} is equivalent to requiring the gradient norm to be bounded by $L$,
	%
	\begin{align}\label{eqn_def_manifold_lipschitz_20}
		\| \nabla_\ccalM f_\theta(x) \| 
		~ =  ~ \lim_{\delta \to 0} ~
		\sup_{ x' \neq x ~:~ d_\ccalM (x,x') \leq \delta} ~
		\frac{|f_\theta(x)-f_\theta(x')|}{d_\ccalM(x,x')}  ~
		~ \leq ~ L , \text{\quad for all~}  x \in \ccalM.
	\end{align}
	%
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

With definition \ref{def_manifold_lipschitz} in place and restricting attention to differentiable functions $f_\theta$ our stated goal of learning functions $f_\theta$ with controlled variability over the manifold $\ccalM$ can then be written as
%
% \begin{align}\label{prob:manifold_lipschitz}
	%   \underset{\phi,\rho\geq 0}{\minimize}  \quad   
	%       & \rho, \\
	%   \text{subject to}  \quad 
	%       & \mbE_{p(x,y)} [\ell \left(\phi(x),y\right)]\leq \epsilon, \nonumber\\
	%       & \| \nabla_\ccalM \phi(z) \|^2 \leq \rho ,\quad z \in \ccalM . \nonumber
	% \end{align}
\begin{align}\label{prob:manifold_lipschitz}
	P^* = \ \ \ \ \ \ \underset{\theta\in\Theta,\rho\geq 0}{\min}  \quad   
	& \rho, \\
	\text{subject to}  \quad 
	& \mbE_{p(x,y)} [\ell \left(f_\theta(x),y\right)]\leq \epsilon, \nonumber\\
	& \| \nabla_\ccalM f_\theta(z) \|^2 \leq \rho ,\quad p(z)\text{-a.e.}, \quad z \in \ccalM . \nonumber
\end{align}
%
In this formulation the statistical loss $\mbE_{p(x,y)} [\ell \left(f_\theta(x),y\right)]$ is required to be below a target level $\eps$. Of all functions $f_\theta$ that can satisfy this loss requirement, Problem \eqref{prob:manifold_lipschitz} defines as optimal the one whose Lipschitz constant $L=\sqrt{\rho}$ is smallest. The goal of this paper is to develop methodologies to solve \eqref{prob:manifold_lipschitz} when the data distribution and the manifold are unknown. To characterize the distribution we are given sample pairs $(x_i,y_i)$ drawn from the joint distribution $p(x,y)$. To characterize the manifold we are given samples $z_i$ drawn from the marginal distribution $p(x)$. This includes the samples $x_i$ from the (labeled) data pairs  $(x_i,y_i)$ and may also include (unlabeled) samples $z_i$.

It is interesting to observe that \eqref{prob:manifold_lipschitz} shows that the problems of manifold regularization \cite{belkin2005manifold, niyogi2013manifold, kejani2020graph, li2022neural} and Lipschitz constant control \cite{oberman2018lipschitz, finlay2018improved,couellan2021coupling, finlay2018lipschitz, pauli2021training, krishnan2020lipschitz, shi2019neural, lindemann2021learning, arghal2021robust} are related. This connection is important to understand the merit of \eqref{prob:manifold_lipschitz}. To explain this better observe that there are three motivations for the problem formulation in \eqref{prob:manifold_lipschitz}: (i) It is often the case that if samples $x_1$ and $x_2$ are close, then the conditional distributions $p(y|x_1)$ and $p(y|x_2)$ are close as well. A function $f_\theta$ with small Lipschitz constant leverages this property. (ii) The Lipschitz constant of $f_\theta$ is \emph{guaranteed} to be smaller than $L=\sqrt{\rho}$. This provides advantages in, e.g., physical systems where Lipschitz constant guarantees translates to stability and safety assurances. (iii) It leverages the intrinsic low-dimensional structure of the manifold $\ccalM$. In particular, this permits taking advantage of unlabeled data. 

Motivations (i) and (ii) are tropes of the Lipschitz regularization literature; e.g., \cite{oberman2018lipschitz, finlay2018improved,couellan2021coupling, finlay2018lipschitz, pauli2021training, krishnan2020lipschitz, shi2019neural, lindemann2021learning, arghal2021robust}. Indeed, the problem formulation in \eqref{prob:manifold_lipschitz} is inspired in similar problem formulations in which the Lipschitz constant is regularized in the ambient space,
%
\begin{align}\label{prob:ambient_lipschitz}
	\underset{\theta\in\Theta,\rho\geq 0}{\minimize}  \quad   
	& L, \\
	\text{subject to}  \quad 
	& \mbE_{p(x,y)} [\ell \left(f_\theta(x),y\right)]\leq \epsilon, \nonumber\\
	&  |f_\theta(y)-f_\theta(z)| \leq L\, \| y - z \|, \quad (y , z)\sim p(x) . \nonumber
\end{align}
%
A difference between \eqref{prob:manifold_lipschitz} and \eqref{prob:ambient_lipschitz} is that in the latter we use a Lipschitz condition that does not require differentiability. A more important difference is that in \eqref{prob:ambient_lipschitz} the Lipschitz constant is regularized in the ambient space. The distance between features $y$ and $z$ in \eqref{prob:ambient_lipschitz} is the Euclidean distance $\| y - z \|$. This is disparate from the manifold metric $d_\ccalM(y,z)$ that is implicit in the manifold gradient constraint in \eqref{prob:manifold_lipschitz}. Thus, the formulation in \eqref{prob:manifold_lipschitz} improves upon \eqref{prob:ambient_lipschitz} because of its ability to leverage the structure of the manifold $\ccalM$ [cf. Motivation (iii)].

Motivations (i) and (iii) are themes of the manifold regularization literature \cite{belkin2005manifold, niyogi2013manifold, kejani2020graph, li2022neural}. And, indeed, it is ready to conclude by invoking Green's first identity (see Section \ref{sec_algorithm}) that the formulation in \eqref{prob:manifold_lipschitz} is also inspired in the manifold regularization problem,
%
\begin{align}\label{prob:manifold_regularization}
	\underset{\theta\in\Theta}{\minimize}  \quad  
	\mbE_{p(x,y)} [\ell \left(f_\theta(x),y\right)] 
	+ \gamma \int_\ccalM \| \nabla_\ccalM f_\theta(z) \|^2 p(z) dV(z).
\end{align}
%
The difference between \eqref{prob:manifold_lipschitz} and \eqref{prob:manifold_regularization} is that in the latter the manifold Lipschitz constant is added as a regularization penalty. This is disparate from the imposition of a manifold Lipschitz constraint in \eqref{prob:manifold_lipschitz}. The regularization in \eqref{prob:manifold_regularization}  \emph{favors} solutions with small Lipschitz constant by penalizing large Lipschitz constants, while the constraint in \eqref{prob:manifold_lipschitz}  \emph{guarantees} that the Lipschitz constant is bounded by $\rho$. This is the distinction between \emph{regularizing} a Lipschitz constant versus \emph{constraining} a Lipschitz constant. The constraint in \eqref{prob:manifold_regularization} is also imposed at \emph{all} points in the manifold, whereas the regularization in \eqref{prob:manifold_regularization} is an average over the manifold. Taking an average allows for large Lipschitz constants at some specific points if this is canceled out by small Lipschitz constants in other points of the manifold. Both of these observations imply that \eqref{prob:manifold_lipschitz} improves upon \eqref{prob:manifold_regularization} because it offers global smoothness guarantees that are important in, e.g., physical systems [cf. Motivation (iii)].

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   R   E   M   A   R   K   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{remark}[Alternative Manifold Lipschitz Control Formulations] \normalfont
	There are three arbitrary choices in \eqref{prob:manifold_lipschitz}. (a) We choose to constrain the average statistical loss $\mbE_{p(x,y)} [\ell \left(f_\theta(x),y\right)]\leq \epsilon$; (b) we choose to constrain the pointwise Lipschitz constant $\| \nabla_\ccalM f_\theta(z) \|^2 \leq \rho$; and (c) we choose as our objective to require a target loss $\eps$ and minimize the Lipschitz constant $L=\sqrt{\rho}$. We can alternatively choose to constrain the pointwise loss $\ell \left(f_\theta(x),y\right)\leq \epsilon$, to constrain the average Lipschitz constant $\int_\ccalM \| \nabla_\ccalM f_\theta(z) \|^2 p_x(z) dV(z) \leq \rho$ [cf \eqref{prob:manifold_regularization}], or to require a target smoothness $L=\sqrt{\rho}$ and minimize the loss $\eps$. All of the possible eight combinations of choices are of interest. We formulate \eqref{prob:manifold_lipschitz} because it is the most natural intersection between the regularization of Lipschitz constants in ambient spaces [cf. \eqref{prob:ambient_lipschitz}] and manifold regularization [cf. \eqref{prob:manifold_regularization}]. The techniques we develop in this paper can be adapted to any of the other seven alternative formulations.
\end{remark}

